Statistical mechanics of a chiral active fluid

Statistical mechanics provides the foundation for describing complex materials using only a few thermodynamic variables. No such framework currently exists far from equilibrium. In this Letter, we demonstrate how thermodynamics emerges far from equilibrium, using fluids composed of active spinners as a case study. Activity gives rise to a single effective temperature that parameterizes both the equation of state and the emergent Boltzmann statistics. The same effective temperature, renormalized by velocity correlations, controls the linear response through canonical Green-Kubo relations for both the familiar shear viscosity and the odd (or Hall) viscosity observed in chiral fluids. The full frequency dependence of these viscosities can be derived analytically by modeling the active-spinner fluid as a random walker undergoing cyclotron motion in shear-stress space. More generally, we provide a first-principles derivation of the Green-Kubo relations valid for a broader class of fluids far from equilibrium. Besides advancing non-equilibrium thermodynamics, our work demonstrates in silico a non-invasive microrheology of active fluids.

==> tex/archive.tex <==
%\begin{abstract}
%Statistical thermodynamics provides us a probabilistic way to describe a matter near equilibrium with just a few macroscopic variables. Applying it to nonequilibrium regime is always a desire but often fails in reality. In this paper, we show the footprints of thermodynamics in a chiral active fluid composed of self-spinning discs that stay far from thermal equilibrium. the system acquires a universal effective temperature in its nonequilibrium steady state and exhibits Boltzmann statistics in both particle kinetics and spatial arrangement. Its linear responses towards small perturbations even obey the fluctuation--dissipation relation, although active spinning breaks both parity and time-reversal symmetries. Moreover, complex fluid flows including shock waves can be fully captured by a modified hydrodynamic theory.
%%Thermodynamics allows us to describe a matter near equilibrium by just a few macroscopic variables. Expanding it to far-from-equilibrium regime is tempting but often intractable in reality. In this paper, we show the footprints of thermodynamics in a chiral active fluid composed of self-spinning discs, which fails in all standard requirements of statistical mechanics. 
%which stays far from equilibrium with broken symmetries in both parity and time-reversal failing in all standard requirements of statistical mechanics. %Nevertheless, the system acquires a universal effective temperature at its nonequilibrium steady state and exhibits Boltzmann statistics in both particle kinetics and spatial arrangement. Linear responses of the fluid even obey the fluctuation--dissipation relation. Moreover, a continuum hydrodynamic theory can be established to capture various complex flows in this chiral active fluid including shock waves. 
%%Nevertheless, the system acquires a universal effective temperature governing both Boltzmann statistics and fluctuation--dissipation relation (FDR). More remarkably, there is a direct mapping between the linear response of this fluid and a chiral Brownian motion in stress space, which naturally expands FDR to dissipationless odd viscosity. Such chiral nature indeed leads to exotic hydrodynamic phenomena such as transverse shock wave, which otherwise are disallowed in common fluids.
%\end{abstract}

%In air, nitrogen, oxygen and other gas molecules constantly collide with each other, rendering a thermal equilibrium. At equilibrium, all microscopic degrees of freedom including molecular velocities and positions follow Boltzmann statistics parameterized with only a few macroscopic variables, temperature $T$, pressure $P$ and etc... Perturbing the air would drive hydrodynamic flows with viscous effects, which dissipate mechanical energy as heat and eventually bring the air back to equilibrium. The viscosity in such transport phenomenon is in fact linked with thermal fluctuations at equilibrium, known as the fluctuation--dissipation relation.
%In air, nitrogen, oxygen and other gas molecules constantly collide with each other, rendering thermal equilibrium. According to statistical thermodynamics, at equilibrium, all microscopic degrees of freedom follow Boltzmann statistics  parameterized with only a few macroscopic variables such as temperature $T$ and pressure $P$. Near equilibrium, perturbing the air drives aerodynamic flows, with transport coefficients determined by the fluctuation--dissipation relation. 
%Perturbing the air would drive hydrodynamic flows that dissipate energy to restore the equilibrium, known as linear responses governed by the fluctuation--dissipation theorem. 
%These thermodynamic principles typically require detailed balances thus cannot be expanded to far-from-equilibrium regime in general. 

%\caption{\label{fig:measurements} \textbf{``Thermal equilibrium'' and linear responses of a chiral active fluid.} \textbf{a.} Schematic of the system setup. We simulate a two-dimensional (2D) granular gas composed of frictional discs self-spinning at a constant angular velocity $\Omega$. Periodic boundary conditions are applied in all dimensions to avoid global rotation. When two spinners collide, they gain transverse motion via interparticle friction. Such collision leads to the emergence of effective temperature as well as odd viscosities. \textbf{b.} Effective temperature. Akin to a thermal gas, this chiral active fluid at equilibrium acquires a Gaussian distribution of particle velocity. An effective temperature $T_\text{eff}$ can be derived from from the velocity variance. Inset: Dependence of $T_\text{eff}$ on $\Omega$. \textbf{c.} Odd stress. Active torque that drives particle self-spinning gives rise to antisymmetric stress, known as odd stress. At equilibrium, it exhibits as a nonvanishing torque density $\tau$, which is linear with $\Omega$ and quadratic with particle density $\rho$. \textbf{d.} Odd and shear viscosities. An oscillatory simple shear invokes shear stress $s_1$ (\protect\so) via odd viscosity $\eta^\text{o}$ and shear stress $s_2$ (\protect\st) via shear viscosity $\eta$. Dependences of $\eta^\text{o}$ and $\eta$ on $\Omega$ are shown by the pink and cyan curves, respectively. \textbf{e.} Rotation and bulk viscosities. An oscillatory dilation/compression corrects $\tau$ (\protect\tor) via rotation viscosity $A$ and pressure $P$ (\protect\p) via bulk viscosity $\zeta$. Dependences of $A$ and $\zeta$ on $\Omega$ are shown in purple and blue, respectively. All quantities are normalized by reduced units ($v_0, t_0, \eta_0, ...$) defined in the Method section.}

%such as emergent edge currents, topologically protected phonon modes and odd (Hall) viscosity. 

%Can a systematic thermodynamic description still exist? If so, how to incorporate FDR with \textit{dissipationless} odd (or Hall) viscosity, one of the most intriguing discoveries in chiral active fluids? Current understanding of chiral active fluids is mostly limited to phenomenological hydrodynamic theories with mean-field approximations, which cannot capture thermal fluctuations. 

Odd viscosity. Active torque that drives particle self-spinning gives rise to a nonvanishing torque density, known as odd stress $\tau$. At the steady state, $\tau = \Gamma(\rho)\Omega \propto \rho^2\Omega$, where $\Gamma$ is the rotational dissipation coefficient and $\rho$ is the particle number density.

%Beyond these common thermal properties, active rotation also contributes odd stress $\tau = \Gamma (\Omega - \omega)$ with $\Gamma$ the rotational diffusion coefficient, a nonvanishing torque density unless the fluid performs a rigid-body rotation with vorticity $\omega = \Omega$.
%Since active rotation injects angular momentum into the system, it contributes an extra property, odd stress $\tau = \Gamma (\Omega - \omega)$ with $\Gamma$ the rotational diffusion coefficient and $\omega$ the vorticity of the fluid. This leads to a nonvanishing torque density at the steady state where $\omega = 0$. 


%It can be rationalized as follow: Odd stress originates from surface friction between two colliding particles and the collision probability in the system scales quadratic with particle density $\rho$. 


%the probability transfer in particle velocity due to interparticle collision $P(\bm{v_1^\text{out}},\bm{v_2^\text{out}} \mid \bm{v_1^\text{in}}, \bm{v_2^\text{in}})$. 


%acting as an effective ``thermostat'' that constantly pumps energy into the system.
%constantly pumping energy into the system.
%We focus on the resultant translational motions of the particles.
%agitated by such effective ``thermostat''.

\begin{subequations}
\begin{eqnarray}
\dot{s}_1 &=& -\gamma s_1 - \gamma^\text{o} s_2 + R_1,
\\
\dot{s}_2 &=& \ \gamma^\text{o} s_1 - \enspace \gamma s_2 + R_2,
\end{eqnarray}
\end{subequations}

\begin{equation}\label{eq:diffusion}
\begin{aligned}
&\dot{s}_1 =-\gamma s_1 - \gamma^\text{o} s_2 + R_1, &
\\
&\dot{s}_2 = \;\gamma^\text{o} s_1 - \gamma s_2 \enspace + R_2,&
\end{aligned}
\end{equation}

\begin{equation}
%\dot{\textbf{S}} = \bm{\Upsilon}\textbf{S} + \textbf{R}
%\frac{\text{d}}{\text{d}t}
\begin{pmatrix} \dot{s}_1 \\ \dot{s}_2 \end{pmatrix} = -\begin{pmatrix} \gamma & \gamma^\text{o} \\ -\gamma^\text{o} & \gamma \end{pmatrix} \begin{pmatrix} s_1 \\ s_2 \end{pmatrix} + \begin{pmatrix} R_1 \\ R_2 \end{pmatrix}
\end{equation}
with damping parameters $\gamma$ and $\gamma^\text{o}$

with damping matrix $\bm{\Upsilon} = \begin{pmatrix} \gamma & \gamma^\text{o} \\ -\gamma^\text{o} & \gamma \end{pmatrix}$ and noise $\textbf{R} = (R_1, R_2)^\text{T}$.

and $\textbf{R} = $


By solving the Langevin equations, we derive time correlation functions $\left<s_1(0)s_1(t)\right>/\left<s_1^2(0)\right> = \text{e}^{-\gamma t} \cos(\gamma^\text{o} t)$ and $\left<s_1(0)s_2(t)\right>/\left<s_1^2(0)\right> = \text{e}^{-\gamma t} \sin(\gamma^\text{o} t)$,
and thus viscosities $\tilde{\eta} = \eta/C = \gamma/(\gamma^2+\gamma^\text{o}^2)$ and $\tilde{\eta}^\text{o} = \eta^\text{o}/C = -\gamma^\text{o}/(\gamma^2+\gamma^\text{o}^2)$ with a  normalization factor $C = A\left<s_1^2(0)\right>/k_\text{B}T_\text{eff}$. 


from mean free path $l$ is and averaged relative velocity $\bar{v}$, $f = 0.5\rho\bar{v}/l$, where $\bar{v}/l$ is the collision frequency of individual particles and one half corrects double counting of the interparticle collisions. 


\author{Ming Han}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Pritzker School of Molecular Engineering,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
 
\author{Michel Fruchart}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Department of Physics, The University of Chicago, Chicago, IL 60637, U.S.A.}

\author{Colin Scheibner}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Department of Physics, The University of Chicago, Chicago, IL 60637, U.S.A.}

\author{Suriyanarayanan Vaikuntanathan}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Department of Physics, The University of Chicago, Chicago, IL 60637, U.S.A.}

\author{William Irvine}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Department of Physics, The University of Chicago, Chicago, IL 60637, U.S.A.}
  
\author{Juan de Pablo}
\affiliation{Pritzker School of Molecular Engineering,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{\fontsize{1}{2}Center for Molecular Engineering, Argonne National Laboratory, Lemont, Illinois 60439, U.S.A.}

\author{Vincenzo Vitelli}
\affiliation{James Franck Institute,
  University of Chicago, Chicago, Illinois 60637, U.S.A.}
\affiliation{Department of Physics, The University of Chicago, Chicago, IL 60637, U.S.A.}



\begin{figure*}[t]
\includegraphics[width=\textwidth]{fluctuation-dissipation4.pdf}
\caption{\label{fig:fluctuations} \textbf{Fluctuation--dissipation relation.} \textbf{a.} Chiral Brownian motion in stress space at $\Omega = 26.7/t_0$. Time evolution of the shear stresses  $\textbf{S} = (s_1, s_2)$ at equilibrium resembles a confined 2D random walk (pink curve in background) turning preferentially clockwise over time (curve with gradient coloring). Inset: Turning angle $\theta (t)$. Such chiral Brownian motion can be modeled as the Langevin dynamics of an effective particle experiencing a radial restoring force \textbf{F}, a tangential rotation force $\textbf{F}^\textbf{o}$, and a noise term \textbf{R} (see the dashed box). Parameters $\gamma = c\eta/(\eta^2+{\eta^\text{o}}^2)$ and $\gamma^\text{o} = -c\eta^\text{o}/(\eta^2+{\eta^\text{o}}^2)$ with normalization factor $c = \rho k_\text{B} T_\text{eff}/A$. \textbf{b.} Stress--stress time correlations. Both simulation measurement and theoretical prediction by the Langevin dynamics model are presented. \textbf{c.} Comparison between measured $\eta^\text{o}$ and theoretical prediction using the Green--Kubo relation. \textbf{d.} Noise--Noise time correlations. Crose time correlations are negligible, and autocorrelations decay over a hundred times faster than that of the stresses (indicated by the dot-dashed lines). Thus the noise term in real simulations can be treated as a 2D white noise.  \textbf{e.} Comparison between measured stress fluctuations and theoretical prediction drawn from the noise term.
}
\end{figure*}

\begin{figure}[t]
\includegraphics[width=0.48\textwidth]{fluctuation-dissipation5.pdf}
\caption{\label{fig:fluctuations} \textbf{Fluctuation--dissipation relation.} \textbf{a.} Stress--stress time correlations at $\Omega = 26.7/t_0$. Simulation measurement and theoretical prediction by the Langevin dynamics model (eq.~\ref{eq:langevin}) are shown as dashed and solid lines, respectively. \textbf{b.} Comparison between measured odd viscosity and theoretical prediction using our modified Green--Kubo formula. \textbf{c.} Chiral Brownian motion in stress space. Time evolution of the shear stresses  $\textbf{S} = (s_1, s_2)$ at the steady state resembles a confined 2D random walk (grey curve in background) turning preferentially clockwise over time (curve with gradient coloring). Inset: Turning angle $\theta (t)$. The chiral Brownian motion can be modeled as the Langevin dynamics of an effective particle driven by a radial restoring force \textbf{F}, a tangential rotation force $\textbf{F}^\textbf{o}$, and a noise term \textbf{R} (see the dashed box). 
}
\end{figure}


\begin{equation}\label{eq:langevin}
%\begin{aligned}
\enspace\enspace \dot{\textbf{S}} = -\bm{\tilde{\eta}}^{-1}\textbf{S} + \textbf{R}  \enspace\enspace \text{with} \enspace \bm{\tilde{\eta}} = c\begin{pmatrix}\eta & \eta^\text{o} \\ -\eta^\text{o} & \eta \end{pmatrix}.
%\end{aligned}
\end{equation}

\begin{equation}\label{eq:langevin}
\begin{aligned}
\dot{\textbf{S}} &= -\bm{\tilde{\eta}}^{-1}\textbf{S} + \textbf{R}  \\ \bm{\tilde{\eta}} &= \frac{ k_\text{B}T_\text{eff}}{A\left<s^2_1(0)\right>}\begin{pmatrix}\eta &  \eta^\text{o} \\ -\eta^\text{o} & \eta \end{pmatrix} \\
\textbf{R} &= \sqrt{\frac{\eta k_\text{B}T_\text{eff}}{A\cdot\text{det}(\bm{\tilde{\eta}})}}\begin{pmatrix} W_1 \\ W_2\end{pmatrix}
\end{aligned}
\end{equation}

\begin{equation}
%\begin{aligned}
\begin{pmatrix}  \dot{s}_1 \\ \dot{s}_2 \end{pmatrix}  = 
- \begin{pmatrix}  \gamma & \gamma^\text{o} \\ -\gamma^\text{o} & \gamma \end{pmatrix} \begin{pmatrix}  s_1 \\ s_2 \end{pmatrix}  +   \sqrt{\gamma\left<|\textbf{S}|^2\right>} \begin{pmatrix}  w_1 \\ w_2 \end{pmatrix}, %\\ &\shortspace \dot{\textbf{S}} \midspace\longspace  -\bm{\gamma}\textbf{S}  \longspace\longspace \textbf{R}
%\end{aligned}
\end{equation}

\begin{equation}\label{eq:langevin}
\begin{split}
\dot{\textbf{S}} = -\bm{\tilde{\eta}}^{-1}\textbf{S} + \textbf{R}, \longspace\longspace\midspace\\
\\
\bm{\tilde{\eta}} = \frac{ k_\text{B}T_\text{eff}}{A\left<s^2_1(0)\right>}\begin{pmatrix}\eta &  \eta^\text{o} \\ -\eta^\text{o} & \eta \end{pmatrix} \shortspace \textbf{R} = \sqrt{\frac{\eta k_\text{B}T_\text{eff}}{A\cdot\text{det}(\bm{\tilde{\eta}})}}\begin{pmatrix} w_1 \\ w_2\end{pmatrix}
\end{split}
\end{equation}


\begin{equation}\label{eq:langevin}
\begin{aligned}
\dot{\textbf{S}} &= -\bm{\tilde{\eta}}^{-1}\textbf{S} + \textbf{R}  \\ 
\shortspace & \longspace\\
\bm{\tilde{\eta}} &= \frac{ k_\text{B}T_\text{eff}}{A\left<s^2_1(0)\right>}\begin{pmatrix}\eta &  \eta^\text{o} \\ -\eta^\text{o} & \eta \end{pmatrix} \\
\textbf{R} &= \sqrt{\frac{\eta k_\text{B}T_\text{eff}}{A\cdot\text{det}(\bm{\tilde{\eta}})}}\begin{pmatrix} W_1 \\ W_2\end{pmatrix}
\end{aligned}
\end{equation}

First, a standard stress--stress correlation analysis is performed on the global pure shear stresses $s_1$ (\protect\so) and $s_2$ (\protect\st) that involve $\eta^\text{o}$ (Fig.~\ref{fig:fluctuations}b).
We find that the autocorrelations $\left<s_1(0)s_1(t)\right> = \left<s_2(0)s_2(t)\right>$. This is owing to the isotropy of the steady state: a $45^\circ$ rotation of the coordinate system swaps $s_1$ and $s_2$ but does not affect the underlying physics of the state.
However, the cross time correlations $\left<s_1(0)s_2(t)\right> = -\left<s_2(0)s_1(t)\right>$. 
The sign change reflects the anti-symmetric nature of odd viscosity (eq.~\ref{eq:matrix}). 
More importantly, it demonstrates that time-reversal symmetry breaks even at the global level. 
Lastly, there is no instantaneous cross correlation $\left<s_1(0)s_2(0)\right> = 0$, validating our independent decomposition of the stress. 

With the stress--stress correlation functions, we can then evaluate fluctuation--dissipation relation using the Green--Kubo formula.
For shear viscosity, $\eta = \int_0^{\infty} \left<s_1(0)s_1(t)\right> \text{d}t \cdot A/k_\text{B}T_\text{eff}$ with $A$ the total area of the system. It agrees well with the linear-response measurements (Supplementary Fig. xx).
For odd viscosity, we propose $\eta^\text{o} = \int_0^{\infty} \left<s_2(0)s_1(t)\right> \text{d}t \cdot A/k_\text{B}T_\text{eff}$, which characterizes how an excitation in stress $s_2$ would induce stress $s_1$ over time.
A similar idea was mentioned in a recent paper as well. Remarkably, this modified Green--Kubo formula gives an excellent prediction on $\eta^\text{o}$ (Fig.~\ref{fig:fluctuations}c).
These findings confirm the existence of fluctuation--dissipation relation as well as expand it for dissipationless odd viscosity. 
In fact, the fluctuation--dissipation relation also holds in frequency domain (Supplementary Fig. xx), making it possible to predict linear response of the chiral active fluid under arbitrary time-varying perturbations.

%It describes a chiral Brownian motion of an effective particle subject to a radial restoring force and a tangential rotating force (Fig.~\ref{fig:fluctuations}a). 

\begin{equation}
\begin{split}
    \sigma_{ij} = \epsilon_{ij} \Gamma(\rho) (\Omega - \omega) - p \delta_{ij} + \eta(\partial_i u_j + \partial_i u_j) + \eta^\text{o}(\partial_i u_j + \partial_i u_j)
\end{split}
\end{equation}


Near equilibrium, thermodynamics allows us to describe materials with only a few macroscopic variables. 
To apply it, time-reversal symmetry in microscopic dynamics is often required. 
Here we show that thermodynamics can be expanded to far-from-equilibrium regime and incorporate nonreciprocal phenomena by relaxing microscopic reversibility.
The concept is demonstrated using a chiral active fluid composed of self-spinning particles.
It acquires a non-equilibrium steady state, exhibiting Boltzmann statistics with a universal effective temperature. 
Owing to broken time-reversal symmetry by self-spinning, the fluid displays chiral linear responses characterized by a dissipationless odd viscosity. 
Interestingly, there is a direct mapping from the steady-state fluctuations of this many-body system to a single-particle chiral Brownian motion in stress space, which naturally expands fluctuation--dissipation relation with odd viscosity.
The presence of odd viscosity indeed leads to exotic hydrodynamic phenomena such as transverse modes in shock wave, which are otherwise disallowed in fluids. 
This nontrivial expansion of thermodynamics relies on the volume conservation of phase space, and can be generalized to a class of active matters where driving forces are decoupled with particle velocities.
